Distributed algorithm for controlling scale-free polygonal formations

This paper presents a distributed algorithm for controlling the deployment of a team of mobile agents in formations whose shapes can be characterized by a broad class of polygons, including regular ones, where each agent occupies a corner of the polygon. The algorithm shares the appealing properties of the popular distance-based rigid formation control, but with the additional advantage of requiring the control of fewer pairs of neighboring agents. Furthermore, the scale of the polygon can be controlled by only one pair of neighboring agents. We also exploit the exponential stability of the controlled formation in order to steer the formation as a whole with translations and rotations in a prescribed way. We provide both theoretical analysis and illustrative simulations.

==> Makefile <==
all: ifac2017_poly.pdf

clean:
	$(RM) *~ *.pdf *.dvi *.log *.aux *.bbl *.blg *.toc *.lol *.loa *.lox \
		*.lot *.out *.lg *.tmp *.xref *.lof .*.swp

ifac2017_poly.pdf: ifac2017_poly.tex
	pdflatex ifac2017_poly
	bibtex ifac2017_poly
	pdflatex ifac2017_poly
	pdflatex ifac2017_poly

